Detection of MeV electrons using a charge integrating hybrid pixel detector

Electrons are emerging as a strong complement to X-rays for diffraction based studies. In this paper we investigate the performance of a JUNGFRAU detector with 320 um thick silicon sensor at a pulsed electron source. Originally developed for X-ray detection at free electron lasers, JUNGFRAU features a dynamic range of 120 MeV/pixel (implemented with in-pixel gain switching) which translated to about 1200 incident electrons per pixel and frame in the MeV region. We preset basic characteristics such as energy deposited per incident particle, resulting cluster size and spatial resolution along with dynamic (intensity) range scans. Measurements were performed at 4, 10 and 20 MeV/c. We compare the measurements with GEANT4 based simulations and extrapolate the results to different sensor thicknesses using these simulations.

==> cluster_table.tex <==



% Simulations
%  320 um sensor 
%  4 MeV 2.30, mean energy: 115 keV
% 10 MeV 1.74, mean energy: 110 keV
% 20 MeV 1.62, mean energy: 111 keV

% Measurements
%  4 MeV 2.46, mean_e: 120 keV
% 10 MeV 1.76, mean_e: 116 keV
% 20 MeV 1.56, mean_e: 112 keV



